Verification of Relational Data-Centric Dynamic Systems with External Services

Data-centric dynamic systems are systems where both the process controlling the dynamics and the manipulation of data are equally central. In this paper we study verification of (first-order) mu-calculus variants over relational data-centric dynamic systems, where data are represented by a full-fledged relational database, and the process is described in terms of atomic actions that evolve the database. The execution of such actions may involve calls to external services, providing fresh data inserted into the system. As a result such systems are typically infinite-state. We show that verification is undecidable in general, and we isolate notable cases, where decidability is achieved. Specifically we start by considering service calls that return values deterministically (depending only on passed parameters). We show that in a mu-calculus variant that preserves knowledge of objects appeared along a run we get decidability under the assumption that the fresh data introduced along a run are bounded, though they might not be bounded in the overall system. In fact we tie such a result to a notion related to weak acyclicity studied in data exchange. Then, we move to nondeterministic services where the assumption of data bounded run would result in a bound on the service calls that can be invoked during the execution and hence would be too restrictive. So we investigate decidability under the assumption that knowledge of objects is preserved only if they are continuously present. We show that if infinitely many values occur in a run but do not accumulate in the same state, then we get again decidability. We give syntactic conditions to avoid this accumulation through the novel notion of "generate-recall acyclicity", which takes into consideration that every service call activation generates new values that cannot be accumulated indefinitely.

==> decidabilitySummary.tex <==
\section{Summary of (Un)decidability Results}
\newcommand{\dec}{\textbf{D}\xspace}
\newcommand{\undec}{\textbf{U}\xspace}
\newcommand{\golu}{\begin{rotate}{90}$\Rsh$\end{rotate}}
\newcommand{\gold}{\begin{rotate}{90}$\Lsh$\end{rotate}}
\newcommand{\gour}{\begin{rotate}{0}$\Rsh$\end{rotate}}
\newcommand{\goul}{\begin{rotate}{90}$\Lsh$\end{rotate}}


\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{R}{>{\raggedleft\arraybackslash}X} 
\newcolumntype{L}{>{\raggedright\arraybackslash}X} 




\begin{table}
\centering
\begin{tabularx}{.8\columnwidth}{R@{~~~~~~}c@{~}c@{~}c@{~}c@{~}c@{~}l}
\multicolumn{7}{c}{\textsc{deterministic services semantics}}\\
\toprule
& $\mu\L$ && \muladom && \mulpers&\\
\midrule
\textsc{unrestricted}  
& \undec & $\leftarrow$
& \undec & $\leftarrow$
& \fbox{\undec} &\\
& $\uparrow$ && && \\
\textsc{bounded run} 
& \fbox{\undec} & 
& \fbox{\dec} & $\rightarrow$
& \dec &\\
\bottomrule
\\
\multicolumn{7}{c}{\textsc{nondeterministic services semantics}}\\
\toprule
& $\mu\L$ && \muladom && \mulpers&\\
\midrule
\textsc{unrestricted}  
& \undec & $\leftarrow$
& \undec & $\leftarrow$
& \fbox{\undec} & \\
& $\uparrow$&&$\uparrow$&&\\
\textsc{bounded state}
& \undec & $\leftarrow$ & \fbox{\undec }& &\fbox{\dec} &\\
%& $\uparrow$&&$\uparrow$&&$\downarrow$\\
%\textsc{bounded run}
%& \undec & $\leftarrow$ & \fbox{\undec} & & \dec &\\
\bottomrule
\end{tabularx}
\end{table}




%%%%% OLD TABLE WITH THREE ROWS FOR THE DET. SEMANTICS %%%%
\iffalse
\begin{table*}
\centering
\begin{tabularx}{\textwidth}{R@{~~~~~~}c@{~}c@{~}c@{~}c@{~}c@{~}L}
\multicolumn{7}{c}{\textsc{deterministic services semantics}}\\
\toprule
& $\mu\L$ && \muladom && \mulpers&\\
\midrule
\textsc{unrestricted}  
& \undec & $\leftarrow$
& \undec & $\leftarrow$
& \fbox{\undec} &\\
& $\uparrow$ && $\uparrow$ && \\
\textsc{bounded state} 
& \undec & $\leftarrow$
& \fbox{\undec} &
& \dec  & \rotatebox[origin=c]{180}{$\hookrightarrow$} (from the table below)\\
& $\uparrow$ &&  && $\downarrow$\\
\textsc{bounded run} 
& \fbox{\undec} & 
& \fbox{\dec} & $\rightarrow$
& \dec &\\
\bottomrule
\\
\multicolumn{7}{c}{\textsc{nondeterministic services semantics}}\\
\toprule
& $\mu\L$ && \muladom && \mulpers&\\
\midrule
\textsc{unrestricted}  
& \undec & $\leftarrow$
& \undec & $\leftarrow$
& \undec & $\hookleftarrow$ (from the table above)\\
& $\uparrow$&&$\uparrow$&&\\
\textsc{bounded state}
& \undec & $\leftarrow$ & \undec & & \fbox{\dec} &\\
& $\uparrow$&&$\uparrow$&&$\downarrow$\\
\textsc{bounded run}
& \undec & $\leftarrow$ & \fbox{\undec} & & \dec &\\
\bottomrule
\end{tabularx}
\end{table*}
\fi



\endinput



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

==> denials.tex <==
\section{Data-Centric Dynamic Systems}
\label{sec:denials}
{\bf Accommodating denial constraints.}

In this appendix, we show how denial constraints can be accommodated inside $\dcds$s.
Let $\sys = \tup{\dl,\pl}$ be a \dcds with data layer
$\dl=\tup{\CONST, \schema, \EC, \idb}$ and process layer $\pl=\tup{\FUNC,\aset,\rset}$.

Let $\Lambda = \{\delta_1,\dots,\delta_n\}$ be a set of \emph{denial
  constraints}. In particular, each $\delta_i$ has the form  $Q_i \ra \false$,
  where $Q_i$ is a domain independent FO query over $\schema$ using constants
  from the active domain $\adom{\idb}$ of $\idb$.

  To encode $\Lambda$ into $\sys$, we augment $\sys$ obtaining
  $\sys_\Lambda = \tup{\dl_\Lambda,\pl_\Lambda}$, where
  $\dl_\Lambda=\tup{\CONST, \schema \cup \{\mathit{Neq}/2\}, \EC \cup
    \EC_\Lambda, \idb \cup \{\mathit{Neq}(a,b)\}}$ and
  $\pl_\Lambda=\tup{\FUNC,\aset_\Lambda,\rset}$, making the assumption
  that $\mathit{Neq}/2$ is a special relation not part of
  $\schema$. $\aset_\Lambda$ is defined as $\aset$, by modifying each
  action specification so as to include persistence of the special
  singleton $\mathit{Neq}(a,b)$ tuple introduced in the initial database of
  $\dl_\Lambda$. This corresponds to an additional effect
  specification $\mathit{Neq}(x,y) \rightsquigarrow \mathit{Neq}(x,y)$. $\EC_\Lambda =
  \{\EC_{\delta_1},\ldots,\EC_{\delta_n}\}$ instead models the denial
  constraints in terms of equality constraints. In particular, given
  $\delta_i = Q_i \ra \false \in \Lambda$, $\EC_{\delta_i}$ represents
  it as follows: $\EC_{\delta_i} = Q_i \land \mathit{Neq}(x,y) \ra x = y$. By
  definition, the singleton $\mathit{Neq}$ tuple exists in every state of \sys,
  and contains two distinct constant values $a$ and $b$. Therefore,
  only those states in which the query $Q_i$ of $\delta_i$ is false
  are kept.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> det-abstract.tex <==

\subsection{Abstract Transition System}
\label{sec:abstract-det}
Given a \dcds $\S = \tup{\dl,\pl}$ with data layer $\dl =
\tup{\CONST,\schema,\EC,\idb}$ and process layer
$\pl=\tup{\FUNC,\aset,\rset}$, we observe that its concrete transition
system $\cts{\sys}$ is typically infinite state. One of the reasons for this
infinite number of states are the actual values produced as result
of external service calls, which belong to an infinite domain
($\CONST$).  However, for verification purposes we are not interested
in such actual values, but only in the possible ways they relate to
each other, by means of equalities and inequalities. 
Following this observation, we define a faithful abstraction of $\cts{\sys}$, which we call \emph{abstract
  transition system}.

Let us first focus on how the states of such abstract transition
system are characterized. The first important difference between the
abstract and the concrete transition system is that in the abstract
system service calls are not evaluated.
Therefore, the current instance of the data layer is now made up of constants in
$\adom{\idb}$ and of terms representing possibly nested service calls, used as placeholders for
their corresponding values. A nested service call represents a service
call whose input parameters are values obtained from other service
calls made in the past. 
%%
For example, term $f(g(a),h(b,c))$ denotes a service call whose input values are the
  results of the service calls denoted by $g(a)$ and $h(b,c)$. 
%%

Even if the actual service call results are not known, the transition
system keeps track of the information needed to discriminate the
case in which two terms are equal from the case in which they
are different (\emph{case analysis}).
%%
For completeness reasons, each pair of terms, especially those
involving service calls, must be related in all the possible ways. For example, given two terms $f(a)$ and $g(a,h(b))$,
  the abstract transition system must consider the case in which $f(a) =
  g(a,h(b))$, and the alternative case in which $f(a) \neq
  g(a,h(b))$. Notice that we make the assumption that $a \neq b$ for
  every two constants $a,b \in \CONST$. Hence equalities will always
  involve at least one term with service calls, i.e., functions in $\FUNC$.

%Given a set $T$ of terms, we call \emph{complete
%  commitment} over $T$ to denote a complete assumption about
%(in)equalities, i.e., for each two service calls $s_1,s_2\in S$ either $s_1=s_2$ or
%$s_1\neq s_2$. 
%%
The semantics of deterministic services requires that service calls with fixed parameters always return
the same result. Therefore, once an (in)equality has been established
between two terms, it must be preserved over time. 

To keep track of all such equalities and inequalities, each state of the abstract transition
system contains an \emph{equality commitment}, i.e., a complete
equality type of all terms encountered so far: for
each pair of such terms, they are either asserted to be equal or
unequal. 
%%
This is done by maintaining a partition of all the terms encountered
so far into equivalence classes.
%%
The other part of the abstract state contains a database instance for
$\schema$ over the representatives of such equivalence classes. 

Formally, an \emph{equality commitment} $\history$ is a well-formed partition.
%
%Given a historical commitment $\history$ and a term $t \in
%\hd{\history}$, the \emph{representative} term of $t$ through
%$\history$ is defined as $\rep{t}{\history}=\history^{-1}([t]_{\phd{\history}})$. Notice that
%$[t]_{\phd{\history}}$ is the cell that contains $t$.
%
%  Given a historical commitment $\history$ and a relational instance
%  $\I$, $\history(\I) = \I [t \mapsto \rep{t}{\history}, t \in
%  \hd{\H}]$. Moreover, we say that, $\history$ is \emph{complete} for $\I$ if
%$\adom{\I} \subseteq \hd{\history}$.
%
An abstract state, or \sstate, is a pair
$\tup{\I, \history}$, where $\I$ is a relational instance of $\schema$ over
  $\repset{\history}$ satisfying each equality constraint in $\EC$,
  and $\history$ is an equality commitment.
The \emph{initial \sstate} is $\tup{\idb,
  \history_0}$, where $\history_0$ partitions $
\adom{\idb}$ into singleton equivalence classes, each containing one constant. Notice
that for each constant $c$ in \adom{\idb}, its representative in
$\history_0$ is $c$ itself.

\begin{example}
\label{exm:abstractstate}
Let $\S = \tup{\dl,\pl}$ be a \dcds with data layer $\dl =
\tup{\CONST,\schema,\EC,\idb}$ and process layer
$\pl=\tup{\FUNC,\aset,\rset}$, where
$\schema = \{P/1,S/2,T/1\}$, $\idb= \{P(a), S(a,b),T(a)\}$ and
$\FUNC=\{f/1,g/1\}$. 
Then the initial \sstate is  $\tup{\idb,\{\{\underline{a}\},\{\underline{b}\}\}}$ and a possible later  \sstate is
$\tup{\I,\history}$, with $\I=\{P(b), S(f(a),g(f(a))\}$ and
$\history = \{\{\underline{a}\},\{\underline{b}, g(a)\},
\{\underline{f(a)},f(b)\},\{\underline{g(f(a))}\}\}$, where we have
underlined the representative of each equivalence class.
\end{example}

Next we define what happens when an action is applied in an
\sstate. For this, given a set of ground facts $E$ such that it
includes only terms in $\terms{\history}$, we denote by $\history(E)$
the instance over $\repset{\history}$ obtained from $E$ by replacing each term with
its corresponding representative in $\history$. More precisely,
$\history(E)$ is the instance $\I  = \{\tup{r_1,\ldots,r_n} \in R \mid
R(t_1,\ldots,t_n) \in E \mbox{ and } r_i = \rep{t_i}{\history}\}$.

Now, let $\S = \tup{\dl,\pl}$ be a \dcds with data layer $\dl =
\tup{\CONST,\schema,\EC,\idb}$ and process layer
$\pl=\tup{\FUNC,\aset,\rset}$.  Let
$\alpha$ be an action in $\aset$ of the form
$\actex{\alpha}(p_1,\ldots,p_m): \set{e_1,\ldots,e_m}$ with
$e_i=\map{q_i^+\land Q_i^-}{E_i}$.  Let $\sigma$ be a substitution for
the input parameters $p_1,\ldots,p_m$ with terms taken from $\HERBRAND$.

To capture what happens when $\alpha$ is executed in an \sstate we
introduce a transition relation $\sexec{\sys}$ between
$\sstate$s, called \emph{abstract execution} of $\alpha\sigma$, such
that $\tup{\tup{\I,\history},\alpha\sigma,\tup{\I',\history'}}
\in \sexec{\sys}$ if the following holds:
 \begin{enumerate}\itemsep=0in\parskip=0in
\item $\sigma$ is a legal parameter assignment for $\alpha$ in state
   $\tup{\I,\history}$ and
 \item $\history' = \RCOMM(\I, \alpha\sigma,\history)$ and
 \item $\I' = \history'(\doo{}{}{\I, \alpha\sigma})$ and
\item $\I'$ satisfies $\EC$,
\end{enumerate}
where $\doo{}{}{}$ is defined as in the concrete transition system, and
$\RCOMM(\I,\alpha\sigma,\history)$ nondeterministically returns a new
equality commitment $\history'$ such that $\terms{\history'}$ is formed by $\terms{\history}$ and
  all the terms occurring in $\doo{}{}{\I, \alpha\sigma})$, and $\history'$ is an extension of $\history$ such that
  $\repset{\history} \subseteq \repset{\history'}$.

Intuitively, $\RCOMM$ constructs an extension of the equality commitment
$\history$ by considering the new terms introduced by the action application. Such terms
are either included in one of the equivalence classes already
contained in $\history$, or assumed to be different than all the already
existing terms, and used to form new equivalence classes. In the
former case, $\history'$ maintains the same
representatives of $\history$ for each extended equivalence class; in
the latter, instead, for any newly introduced equivalence class in
$\history'$, a new term is elected as representative among those of
the equivalence class.\\

\noindent \textbf{Abstract transition system.}
Let $\sys = \tup{\dl,\pl}$  be a \dcds  with data layer
$\dl=\tup{\CONST, \schema, \EC, \idb}$ and process layer
$\pl=\tup{\FUNC,\aset,\rset}$.
The \emph{abstract transition system} of $\sys$  is $\sts{\sys} = \tup{\HERBRAND, \R, \Sigma,
    s_0,\db,  \Longrightarrow}$ where $s_0 = \tup{\idb, \history_0}$, and $\db$ is such that $\db(\tup{\I,\history}) = \I$.
Specifically, we define by simultaneous induction $\Sigma$ and $\Longrightarrow$
as the smallest sets satisfying the following properties: \myi  $s_0
\in \Sigma$; \myii  if $\tup{\I,\history} \in \Sigma$ , then for all $Q\mapsto \alpha
  \in \rset$ and all substitutions $\sigma$ for the input parameters
  of $\alpha$ such that $\sigma\in\ans{Q,\I}$, and for every
  $\tup{\I',\history'}$ such that
  $\tup{\tup{\I,\history},\alpha\sigma,\tup{\I',\history'}}\in\sexec{\sys}$,
  we have that $\tup{\I',\history'}\in\Sigma$, and $\tup{\I,\history} \Longrightarrow \tup{\I',\history'}$.

Intuitively, to define the abstract transition system of a \dcds \sys we start from the
initial \sstate $s_0=\tup{\idb,\history_0}$, and for each rule
$\carule{Q}{\alpha}$ in $\pl$, we evaluate $Q$ over $\idb$, and calculate all $\sstate$s
$s$ such that $\tup{s_0,\alpha\sigma,s} \in
\sexec{\sys}$, where $\sigma \in \ans{Q,\idb}$. Then we repeat the same steps considering each $s$,
and so on.
The computation of successor states is done by picking each newly
introduced service call and deciding whether to insert it into an
already existing equivalence class, or to create a new equivalence
class with it. All the successors that violate some equality
constraints are filtered away. Notice that, at each step, only a
finite number of terms are introduced, and hence only
finitely many equality commitments can be placed over them,
giving raise to a finite number of successors. In other words,
$\sts{\sys}$ is \emph{finite branching}.\label{remark:finitebranching}
Notice that, however, the abstract transition system can be anyway infinite, since new terms
could continuously be added.

\begin{example}
Consider the \dcds \sys described in Ex.\ \ref{ex:openruntime}. The
initial active domain is constituted by the single value $a$.  The application of action $\alpha$ in the initial states involves the two
service calls $f(a)$ and $f(g)$. Hence, while the concrete transition
system $\cts{\sys}$ introduces infinitely many successors in which all
the possible values are picked for the two calls, the abstract
transition system $\sts{\sys}$ only contains $5$ successors, which
cover all the complete equality commitments that can be made over $\{a, f(a),
g(a)\}$ (see also Figure~\ref{fig:openRS-abstract}).
\end{example}

%\mrem{Fig.~\ref{fig:openRS-abstract} shows the abstract transition system
%corresponding to the concrete transition system of
%Fig.~\ref{fig:openRS}, which is generated by the \dcds
%introduced in Ex.~\ref{ex:openruntime}.
%Fig.~\ref{fig:openRS-abstract-ec} shows instead the abstract transition system
%corresponding to the concrete transition system of
%Fig.~\ref{fig:openRS-ec}, which is generated by the \dcds
%introduced in Ex.~\ref{ex:openruntime-ec}.}

There is an intimate connection between the concrete and the abstract
transition system of a \dcds. On the one hand, the concrete transition
system issues new service calls and then keeps their values along its evolution
to ensure their deterministic behavior. On the other hand,
the abstract transition system builds equality commitments over the
encountered service calls, and keeps such commitments to ensure their
deterministic behavior. Such an intimate connection is technically
supported by the following theorem:
\begin{theorem}
\label{thm:openbisim}
Given a \dcds \sys with
deterministic services, its concrete and abstract transition systems are
history preserving bisimilar, i.e., $\sts{\sys} \hbsim \cts{\sys}$.
\end{theorem}
A distinctive feature of $\sts{\sys}$ is that it is
finite branching by construction. Furthermore, run-boundedness is
preserved by history preserving bisimulation. The combination of these
two properties leads to our main result for deterministic services:

\begin{theorem}
\label{thm:finitestate-det}
Given a run-bounded \dcds \sys with deterministic services, its abstract transition system $\sts{\sys}$
is finite state. 
\end{theorem}

\begin{theorem}
\label{thm:propositional-det}
Verification of \muladom properties for run-bounded $\dcds$s with
deterministic services  
%Given a run-bounded \dcds \sys with deterministic services and a
%\muladom property $\Phi$, the verification problem $\cts{\sys} \models \Phi$
can be reduced to conventional finite state model checking of propositional $\mu$-calculus. 
\end{theorem}


Theorem~\ref{thm:propositional-det} is directly obtained from Theorems
\ref{thm:finitestate-det} and \ref{thm:openbisim}. In particular, Theorem \ref{thm:openbisim} implies that, given a \dcds \sys, $\cts{\sys}$
and $\sts{\sys} =
\tup{\HERBRAND,\schema,\Sigma,s_0,\db,\Longrightarrow}$ satisfy the same \muladom formulae,
making it possible to use $\sts{\sys}$ in place of $\cts{\sys}$ for
verification. Therefore, given a \muladom property $\Phi$, the
verification problem is reduced to $\sts{\sys} \models \Phi$.
Under the assumption that \sys is run-bounded, Theorem
\ref{thm:finitestate-det} guarantees that $\sts{\sys}$ is finite state.
Let $\adom{\sts{\sys}} = \bigcup_{s_i \in \Sigma} \adom{\db(s_i)}$.
If $\sts{\sys}$ is finite state, then there exists a bound $b$ such
that $|\adom{\sts{\sys}|} < b$. Consequently, it is possible to
transform $\Phi$ into an equivalent \emph{finite} propositional
$\mu$-calculus formula $\prop{\Phi}$, where $\prop{\Phi}$ is
inductively defined over the structure of $\Phi$ leaving it unaltered,
except for the following case: $\prop{\exists x.\inadom(x)\land \Psi(x)} = \bigvee_{t_i \in
  \adom{\sys}} \inadom(t_i) \land \prop{\Psi(t_i)}$.
Clearly, $\sts{\sys} \models \Phi$ if and only if $\sts{\sys} \models
\prop{\Phi}$.

It is well-known that verification of propositional $\mu$-calculus
formulae over finite transition systems is decidable \cite{Emer96},
and therefore Theorem \ref{thm:propositional-det} directly implies
decidability of verification for run-bounded $\dcds$s with
deterministic services.

\begin{corollary}
\label{cor:decidability-det}
Verification of \muladom properties for run-bounded $\dcds$s with
deterministic services is decidable.
\end{corollary}





\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

==> det-verification-results.tex <==
\subsection{Verification Results}\label{sec:det-results}
We now study the verification of $\dcds$s with deterministic
services. In particular, we are interested in the following problem:
given a \dcds \sys and a temporal property $\Phi$, check whether 
$\cts{\sys} \models \Phi$. Not surprisingly, given the expressive power of \dcds\ as a computation model, the verification problem
is undecidable for all $\mu$-calculus logics mentioned in Section~\ref{sec:verif}.
In fact, we can show an even stronger undecidability result,  for a very small fragment of propositional linear temporal logic (LTL)~\cite{ltl-citation}, 
namely the safety properties of the form $G p$ where $p$ is propositional.

\begin{theorem}\label{thm:ltl-undecid-det}
There exists a \dcds\ \sys\ with non-deterministic services, and a propositional safety property $\Phi \in$ LTL,
such that checking $\cts{\sys} \models \Phi$ is undecidable.
\end{theorem}

Since we are interested in verifying non-trivial temporal properties 
(i.e.\ with temporal operators, branching time, and quantification over individuals across time), 
we need to consider restricted classes of $\dcds$s. 
The challenge is to find an acceptable trade-off between expressive power of the class of properties
versus the restricted class of \dcds. From the property side, we restrict the
class of properties to the history preserving logic $\muladom$  seen
in Section~\ref{sec:mula}; notice that this logic is not propositional, it is branching-time
aware, and contains both kinds of immediate successor temporal operators and their fixpoint.
From the \dcds side, we isolate a notable class of ``run-bounded''
$\dcds$s for which verification of $\muladom$ properties is
decidable.
\\


\noindent
{\bf Run-bounded \dcds.}
Let us consider a transition system $\mf{} = \tup{\Delta, \R, \Sigma, s_0, \db,
  \Rightarrow}$. A \emph{run} $\tau$ in $\mf{}$ is a (finite or infinite)
sequence of states rooted at $s_0$: $\tau = s_0s_1s_2\ldots$, where
$s_i \Rightarrow s_{i+1}$. Given such a run, we use $\tau(i)$ to
denote its $i$-th state, and $\tau[i]$ to
represent its finite prefix $s_0 \ldots s_i$.

A run $\tau$ is \emph{(data) bounded} if the number of values mentioned
inside its databases is bounded, i.e., there exists a finite bound
$b$ such that $| \bigcup_{s \textrm{ state of } \tau} \adom{\db(s)}| < b$.
This is equivalent to say that for every finite prefix $\tau[i]$ of $\tau$,
$| \bigcup_{j \in \{0,\ldots,i\}} \adom{\db(s_j)}| < b$.
We say that $\mf{}$ is \emph{run-bounded} if there exists a bound $b$ such that every
run in $\mf{}$ is (data) bounded by $b$. A \dcds \sys is
run-bounded if its concrete transition system $\cts{\sys}$ is run-bounded.
\mrem{Better explain the intuition behind run boundedness, and why it
  isolates an interesting class of DCDSs}
Intuitively, (data) unbounded runs represent executions of the \dcds
in which infinitely many distinct values occur because infinitely many
different service calls are issued. This can only happen when the results
produced by some service calls are then fed into new calls of the same
services, and so on. In other
words, the values of such runs
indirectly depend on arbitrarily many states in the past. Notice that
run boundedness does not impose any restriction about the branching of
the transition system; in particular, $\cts{\sys}$ is typically
infinite-branching because new service calls may return any
possible result.

We are now ready to state our main decidability result for
deterministic services.

\begin{theorem}
\label{thm:det-decidability}
Verification of \muladom properties over run-bounded \dcds with
deterministic services is decidable.
%Given a \dcds \sys and a \muladom formula $\Phi$, if the concrete
%transition system $\cts{\sys}$ is run-bounded, then it is decidable to
%verify whether $\cts{\sys}\models\Phi$.
\end{theorem}

Observe that run-boundedness is a semantic restriction. A natural
question that consequently arises is if it is possible to check
whether a given \dcds is run-bounded. We provide a negative answer to
this question.

\begin{theorem}
\label{thm:det-boundedness}
Checking run-boundedness of $\dcds$s is undecidable.
\end{theorem}

To mitigate this issue, we investigate a sufficient syntactic condition that can
be effectively tested over a \dcds to check whether it is run-bounded.
To do so, we recast the approach of
\cite{Bagheri2011:Artifacts} in the more abstract and expressive framework here presented.
In particular, we first introduce the ``positive approximate'' of a \dcds, which abstracts away some aspects of \sys.
Technically, given a \dcds $\sys = \tup{\dl,\pl}$ with data layer
$\dl=\tup{\CONST, \schema, \EC, \idb}$ and process layer $\pl=\tup{\FUNC,\aset,\rset}$,
its \emph{positive approximate}  $\pos{\sys}$ is a \dcds
$\tup{\pos{\dl},\pos{\pl}}$, where $\pos{\dl}=\tup{\CONST, \schema,
  \emptyset, \idb}$  corresponds to
$\dl$ without equality constraints, while $\pos{\pl} =
\tup{\FUNC,\pos{\aset},\pos{\rset}}$ is a process layer whose actions
$\pos{\aset}$ and process $\pos{\rset}$ are obtained as follows:
\begin{itemize}\parskip=0in\itemsep=0in
\item Each condition-action rule $\carule{Q}{\alpha}$ in $\rset$ becomes
 $\carule{\true}{\pos{\alpha}}$ in $\pos{\rset}$. $\pos{\rset}$ is therefore a process that supports
  the execution of every action in $\pos{\aset}$ at each step.
\item Each action $\alpha(p_1,\ldots,p_n) : \{e_1,\ldots,e_m\}$ in
  $\aset$ becomes $\pos{\alpha} : \{\pos{e_1},\ldots,\pos{e_m}\}$ in
  $\pos{\aset}$, where each $e_i = \map{q_i^+\land   Q_i^-}{E_i}$ becomes in turn $\pos{e_i} =
\map{q_i^+}{E_i}$. Intuitively, the positive approximate action is
obtained from the original action by removing all the parameters from
its signature, and by removing all ``negative'' components from the
query used to instantiate its effect specifications; note that the variables
of $q_i^+$ that were parameters in $\alpha$ are now free variables in $\pos{\alpha}$.
\end{itemize}
The positive approximate obeys the following key property.
\begin{lemma}
Given a \dcds \sys, if the positive approximate $\pos{\sys}$ of \sys is run
bounded, then \sys is run bounded as well.
\end{lemma}
The property attests that proving run boundedness of $\pos{\sys}$ is a
sufficient condition for showing that $\sys$ is run bounded. To prove
run boundedness of the positive approximate, we follow the line of
\cite{BPM2011}, exploiting the strict correspondence between the execution of an action in $\pos{\pl}$ and a step in the chase of
a set of tuple generating dependencies (TGDs) in data
exchange\cite{AbHV95,Kolaitis05:Exchange}.

In particular, we resort to a well-known result in data exchange,  namely chase
  termination for \emph{weakly acyclic} TGDs
  \cite{Kolaitis05:Exchange}. In our setting, the weak acyclicity of 
 a process layer is checked over a dataflow graph constructed by
  analyzing the corresponding positive approximate process
  layer. In particular, given a \dcds $\sys = \tup{\dl,\pl}$  and its positive
  approximate $\pos{\pl} = \tup{\pos{\dl},\pos{\pl}}$, the
  \emph{dependency graph} of $\pos{\pl}$ is an edge-labeled
directed graph $\tup{N,E}$ where: \myi $N \subseteq \schema \times \mathbb{N}^+$ is a set of nodes such
  that $\tup{R,i} \in N$ for every $R/n \in \schema$ and every $i \in
  \{1,\ldots,n\}$; \myii $E \subseteq N \times N \times \{\true,\false\}$ is a set of
  labeled edges where
  \begin{itemize}\parskip=0in\itemsep=0in
    \item an ordinary edge $\tup{\tup{R_1,j},\tup{R_2,k},\false} \in E$ if there exists an action
      $\pos{\alpha} \in \pos{\aset}$, an effect $\map{q_i^+}{E_i}
      \in \effect{\pos{\alpha}}$ and a variable $x$ such that
      $R_1(\ldots,t_{j-1},x,t_{j+1},\ldots)$ occurs in $q_i^+$ and
      $R_2(\ldots,t'_{k-1},x,t'_{k+i},\ldots)$ occurs in
      $E_i$;
    \item a special edge $\tup{\tup{R_1,j},\tup{R_2,k},\true} \in E$ if there exists an action
      $\pos{\alpha} \in \pos{\aset}$, an effect $\map{q_i^+}{E_i}
      \in \effect{\pos{\alpha}}$ and a variable $x$ such that
      $R_1(\ldots,t_{j-1},x,t_{j+1},\ldots)$ occurs in $q_i^+$,
      $R_2(\ldots,t'_{k-1},t,t'_{k+i},\ldots)$ occurs in $E_i$, and
      $t = f(\ldots,x,\ldots)$, with $f \in \FUNC$.
  \end{itemize}
$\pl$ is \emph{weakly acyclic} if the dependency
graph of its approximate $\pos{\pl}$ does not contain any cycle going
through a special edge. We say that a \dcds is weakly acyclic if its
process layer is weakly acyclic.

Intuitively, ordinary edges represent the possible propagation (copy)
of a value across states: $\tup{\tup{R_1,j},\tup{R_2,k},\false} \in E$
means that it could be possible that the value currently stored inside the $j$-th
component of an $R_1$ tuple could be moved to the $k$-th component
of an $R_2$ tuple in the next state. Contrariwise, special edges
represent that a value can be taken as parameter of a service call,
thus contributing to the creation of (possibly new) values across
states: $\tup{\tup{R_1,j},\tup{R_2,k},\true} \in E$ means that the
value currently stored inside the $j$-th component of an $R_1$ tuple
could contribute to generate a (possibly new) value that is then
stored inside the $k$-th component of an $R_2$ tuple.

A cycle going through a special edge represents that the (new) value
obtained by calling a service could be later on used as parameter for
another call of the same service. This  self-dependency may
potentially lead to an infinite number of calls of the same service
along an execution of the system, thus making it impossible to put a
bound on the data accumulated during the run. 


\begin{example}
\label{ex:nonwa}
Let $\sys = \tup{\dl,\pl}$ be a \dcds with data layer
$\dl=\tup{\CONST, \schema, \emptyset, \idb}$ and process layer $\pl=\tup{\FUNC,\aset,\rset}$,
where $\FUNC = \{f/1\}$, $\schema = \{R/1, Q/1\}$, $\EC = \emptyset$, $\idb =
\{R(a)\}$, $ \rset = \{true
\mapsto \actex{A}\}$ and
\begin{align*}
  \actex{A}: ~ \{~R(x) & \rightsquigarrow{Q(f(x))} \\
 Q(x) & \rightsquigarrow{R(x)} ~\}
\end{align*}
\noindent Figure \ref{fig:dgraph-cyclic}
attests that \sys is not weakly acyclic, and
Figure\ref{fig:nonwa-concrete} shows the resulting concrete
transition system $\cts{\sys}$, which is not run-bounded. Notice that,
in this case, the positive approximate of \sys coincides with \sys
itself. Starting from the initial state, $\actex{A}$ calls $f(a)$ and
stores the result inside $Q$. A second
execution of $\actex{A}$ transfers the result of $f(a)$ into $R$. When
$\actex{A}$ is executed for the third time, $f$ is called
again, but using as parameter the previously obtained
result. Consequently, it could be the case that $f$ returns a
new result, because $f(f(a)$ may be
different from $f(a)$. This chain can be repeated forever, leading to
continuously call $f$ every time with a fresh value, possibly generating infinitely many
distinct results along the run.
\end{example}
%%
The absence of cycles going through a special edge guarantees instead
that the \dcds can be effectively verified.
\begin{theorem}
\label{thm:weak-acyclicity}
Any weakly acyclic \dcds is run-bounded.
\end{theorem}
%%
Theorem~\ref{thm:det-decidability} and~\ref{thm:weak-acyclicity} together
imply:
\begin{theorem}
\label{thm:synt-decidability-det}
Verification of \muladom properties for weakly acyclic \dcds with
deterministic services is decidable.
\end{theorem}
Figure \ref{fig:dgraph-acyclic} shows an example of (weakly acyclic)
dependency graph built for the \dcds described in Ex.\
\ref{ex:openruntime}. The weak acyclicity of this graph ensures that
both concrete transition systems depicted in Figure~\ref{fig:openRS}
and \ref{fig:openRS-ec} are run-bounded and, in turn, can be
effectively verified against \muladom properties.




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> nondet-examples.tex <==
\section{Nondet examples}

\arem{to be merged into proper appendix}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> preliminaries.tex <==
 \section{Preliminary Notions}
\arem{If the abstract transition systems sections go to appendix, then most of this also goes to appendix}

We consider a countably infinite set of \emph{constants} $\CONST$, and a 
countably infinite set of \emph{functions} $\FUNC$, each with its own arity greater than or equal to 0. 
%%
We consider also the countably infinite set of \emph{terms} $\HERBAND$
built using $\CONST$ and $\FUNC$. This is the so-called \emph{Herbrand
  universe} obtained from $\CONST$ and $\FUNC$.
%%
We  use the function $\subterms:
\HERBRAND \ra 2^{\HERBRAND}$ to specify the \emph{subterms} of a
term. Such a function is inductively defined as follows:  for each constant $c \in \C$, $\subterms(c)
= \set{c}$, and for each term $f(t_1, \dots, t_n)$,
$\subterms(f(t_1, \dots, t_n))= \set{f(t_1, \dots, t_n), t_1, \dots, t_n} \cup \subterms(t_1) \cup
\dots \cup \subterms(t_n)$.
%%
A set $S$ is \emph{closed under sub-terms} if  for each $\ t\in
\terms{S}$ it holds that
$\subterms(t)\subseteq\terms{S}$. 


\medskip

Given a (finite/infinite) set of terms $S\subseteq\HERBAND$, we can get a 
\emph{partition} $\PART{}$ of $S$ into equivalence classes, also called \emph{cells}, such that two terms in the
same cell of the partition are asserted to be equal, while two terms in two distinct cells are asserted to be different.
%%
Given such a partition $\PART{}$, we can reconstruct the set $S$ that
has been partitioned by considering all the terms appearing in all
cells of $\PART{}$, namely $\terms{\PART{}}=\set{t \in \HERBRAND ~\vert~
  \exists \ec\in\PART{}, t\in ec}$. This allows us to talk about
a partition without mentioning the set it is a partition of.
%%
Given a partition $\PART{}$, and a term $t\in\terms{\PART{}}$, we
denote by $[t]_{\PART{}}$ the equivalence class/cell to which $t$
belongs. When clear from the context we simply use $[t]$ instead of
$[t]_{\PART{}}$.
%%
Given a partition $\PART{}$ and a term $t \in \terms{\PART{}}
$, we assume to have a function $\rep{t}{\PART{}}$ that returns a
\emph{representative} $r$ for the equivalence class to which $t$
belongs. The representative $r$ is one of the elements of
$[t]_\PART{}$; the details on how to choose such a representative are
irrelevant for what follows. We denote by $\repset{\PART{}}$ the set
of representatives of $\PART{}$.
%%
\begin{example}
  \label{exm:partition} Consider $\CONST=\set{a, b}$ and
  $\FUNC=\set{(f,2)}$. $\HERBAND$ is therefore $\set{a, b, f(a,a), f(a,b),
    f(b,a), f(b,b), f(f(a,a), a), \dots}$. One possible partition of
  $\HERBAND$ is $\PART{}=\set{\set{a,f(a,a)}, \set{b}, \set{f(a,b)},
    \dots}$. Notice that $[a]_{\PART{}}=[f(a,a)]_{\PART{}}$
  and $\rep{a}{\PART{}} = \rep{f(a,a)}{\PART{}} = a$ (the latter is
  chosen randomly as the representative of the equivalence class). Furthermore, 
  $\subterms(f(f(a,a),b))=\set{a, b, f(a,a), f(f(a,a),b)}$.
\end{example}
In fact, typically, we are not interested in
every partition but only in those that are well-formed.  
A partition
$\PART{}$ is \emph{well-formed} if: \myi each equivalence class
$ec\in\PART{}$ contains at most one constant $c \in \CONST$, and \myii
$\PART{}$ is \emph{closed-under-congruence}, i.e., for
  each pair $f(t_1, \dots, t_m), f(t^\prime_1, \dots, t^\prime_m)\in
  \terms{\PART{}}$, if $t_i,t'_i \in \terms{\PART{}}$ and $[t_i]_{\PART{}} =
  [t^\prime_i]_{\PART{}}$ for $i\in\{1,\ldots,m\}$, then
  $[f(t_1, \dots, t_m)]_{\PART{}} = [f(t^\prime_1, \dots,
  t^\prime_m)]_{\PART{}}$.
Well-formed partitions reflect the fact that we are enforcing the unique
name assumption on constants, as usual in databases, and the semantics
of functions, which, given the same arguments, return the same values.
%Notice that  \myi implies that distinct constants are always considered different in well formed partitions. Instead \myii is really a requirement on the set $S$ we are partitioning: we do require that such a set includes all the subterms of the terms in it.
%%
If not mentioned explicitly, by a partition we mean a well formed partition. 



Given $S_1,S_2 \subseteq \HERBAND$ such that $S_1 \subseteq S_2$, and
two partition $\PART{}_1$ and $\PART{}_2$ respectively of $S_1$ and
$S_2$, we say that $\PART{}_2$ is an \emph{extension} of $\PART{}_1$,
if there exists an injective function $h: \PART{}_1 \rightarrow \PART{}_2$
such that for each cell $ec\in \PART{}_1$, we have that $ec \subseteq
h(ec)$. In other words each equivalence class $ec$ of $\PART{}_1$ is
completely contained in one of the equivalence classes of $\PART{}_2$,
as a result all equalities and inequalities forming the equivalence classes of $\PART{}_1$ are preserved in $\PART{}_2$.
%%
 In this case, also the
inequalities between distinct equivalence classes in $\PART{}_1$ are
preserved in $\PART{}_2$.
In the special case where $h$ is also bijective, we say $\PART{}_1$
is \emph{embedded in} $\PART{}_2$.
%%
We sometime refer to $h$ as a witness of extension (embedding).


\medskip

Given a first order query $Q$ and a relational instance $\I$, the answer to the query
$\ans{Q,\I}$ is the set of assignments from the free variables of $Q$ to
the domain of $\I$, such that an assignment $\theta\in
\ans{Q,\I}$ if and only if $\I\models Q\theta$. We treat $Q\theta$ as
a boolean query, and with a little abuse of notation, we say
$\ans{Q\theta,\I} \equiv \true$ if and only if $\I\models Q\theta$.
\medskip

%%%GGG Put as a footnote on muLa bisimulation.
Given a partial function $f: S\rightarrow S'$, we denote with $\domain{f}$ the
domain of $f$, i.e., the set of elements in $S$ on which $f$ is defined, and with
$\image{f}$ the image of $f$, i.e., the set of elements $s'$ in $S'$ such that $s'=f(s)$ for some $s\in S$.

%%%GGG Put as a footnote on muLp bisimulation.
% Also, given a set $D$, we denote by
% $\restrict{f}{D}$ the \emph{restriction} of $f$ over the domain
% $\domain{f} \cap D$, i.e.,
% $\domain{\restrict{f}{D}(x)} = \domain{f} \cap
% D$, and
% $\restrict{f}{D}(x)
% = f(x)$ for every $x \in \domain{f} \cap D$.


\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:
